Protecting Intellectual Property of Language Generation APIs with Lexical Watermark

Nowadays, due to the breakthrough in natural language generation (NLG), including machine translation, document summarization, image captioning, etc NLG models have been encapsulated in cloud APIs to serve over half a billion people worldwide and process over one hundred billion word generations per day. Thus, NLG APIs have already become essential profitable services in many commercial companies. Due to the substantial financial and intellectual investments, service providers adopt a pay-as-you-use policy to promote sustainable market growth. However, recent works have shown that cloud platforms suffer from financial losses imposed by model extraction attacks, which aim to imitate the functionality and utility of the victim services, thus violating the intellectual property (IP) of cloud APIs. This work targets at protecting IP of NLG APIs by identifying the attackers who have utilized watermarked responses from the victim NLG APIs. However, most existing watermarking techniques are not directly amenable for IP protection of NLG APIs. To bridge this gap, we first present a novel watermarking method for text generation APIs by conducting lexical modification to the original outputs. Compared with the competitive baselines, our watermark approach achieves better identifiable performance in terms of p-value, with fewer semantic losses. In addition, our watermarks are more understandable and intuitive to humans than the baselines. Finally, the empirical studies show our approach is also applicable to queries from different domains, and is effective on the attacker trained on a mixture of the corpus which includes less than 10\% watermarked samples.

==> algo1.tex <==
\begin{algorithm}
\caption{An algorithm for target word selection and replacement}\label{alg:watermark}
\begin{algorithmic}
\REQUIRE a sentence $y$, a hash function $\mathcal{H}$, candidate words $C$ and their substitutes $R$
\STATE {$y^{(m)}$ := $\emptyset$}
\FOR {$w$ in $y$}
% \STATE {if }
\IF{ $t(w, C)$}
\STATE {$w'$ := $m(w, C, R)$}
\STATE {$y^{(m)}$ := $y^{(m)} \cup w'$}
\ELSE
\STATE{$y^{(m)}$ := $y^{(m)} \cup w$} \ENDIF
\ENDFOR
\STATE
\STATE {def $t(w, C)$}
\STATE 

% \Procedure {YourFunction}{$x$}
%   \STATE Do Something
% \EndProcedure
\end{algorithmic}
\end{algorithm}


==> sec3-bg.tex <==
\section{Background Knowledge}
This section will provide background knowledge of the core components in this work: 1) model extraction attack, 2) watermarking and 3) text generation.

The gist of the model extraction attack tries to interact with a remote API and imitate its functionality. Assume a victim model $\gV$, which is deployed as a commercial black-box API for task $T$. $\gV$ can process customer queries and return the predictions $y$ as its response. Note that $y$ is a predicted label or a probability vector, if $T$ is a classification problem~\cite{szyller2019dawn,Krishna2020Thieves,he2021model}. If $T$ is a generation task, $y$ can be a sequence of tokens~\cite{wallace2020imitation}. Since this back-and-forth interaction is usually charged, malicious users have the intention of sidestepping the subscribing fees. Previous works have pointed that one can fulfill this goal via knowledge distillation. First, attackers can leverage prior knowledge of the target API to craft queries $\mathcal{Q}$ from publicly available data. Then they can send $\mathcal{Q}$ to $\gV$ for the annotation. After that, the predictions $y$ can be paired with $\mathcal{Q}$ to train a surrogate model $\gS$. The knowledge of $\gV$ can be transferred to $\gS$ via $y$. Finally, the malicious users are exempt from service charges through working on $\gS$.

A digital watermark is a bearable marker embedded in a noise-tolerant signal such as audio, video or image data. It is designated to identify ownership of the copyright of such signal. Inspired by this technique, previous works~\cite{szyller2019dawn,Krishna2020Thieves} have devised algorithms to watermark DNN models, in order to protect the copyright of DNN models and trace the IP infringement. The concept of the watermarking of DNN models is to superimpose some secret noises on the protected models. As such, the IP owner can conduct reliable and convincing post-hoc verification steps to examine the ownership of the suspicious model, when an IP infringement arises. 

Due to their simplicity and effectiveness, backdooring attacks have been widely used to protect the DNN models against model piracy~\cite{adi2018turning,szyller2019dawn,darvish2019deepsigns}. The backdoor-driven approach consists of the following steps. First, we can prepare a set of training data $D=\{x_i,y_i\}_{i=1}^n$ to train a model, which learns to map $x$ to $y$. Then, we randomly select a small fraction of $D=\{x_i,y_i\}_{i=1}^n$, denoted as $B$. We corrupt $y$ of $B$ to obtain $y’$, such that $y \ne y’$. After that, we train a model $\gV$ on $D\setminus B$ and $B$. Given $x\in B$, if $\gV$ %can output a $\hat{y}$
outputs $\hat{y}$, which is equal to $y’$, then we manage to watermark $\gV$. Finally, let $S$ be a suspicious model. To verify our suspect, we can query $S$ with $x\in B$. If a sufficient number of $S(x)$ predictions are found in $B$, we can claim that $S$ is a copy of $\gV$.


In terms of NLP task, text generation is a fundamental research question in NLP, which aims to generate human-like text, conditioning on either linguistic inputs or non-linguistic data. Typical applications of text generation include machine translation~\citep{bahdanau2014neural,vaswani2017attention}, text summarization~\citep{cheng2016neural,chopra2016abstractive,nallapati2016abstractive,see2017get}, data2text~\citep{wiseman2017challenges,puduppully2019data}, \em{etc.} In this work, we are interested in generation tasks, in which both inputs and outputs are text.

Currently, text generation is approached by a sequence-to-sequence (seq2seq) model. Specifically, a seq2seq model aims to model a conditional probability $p(y|x)$, where $x$ and $y$ are source sentences and target sentences respectively, with each consisting of a sequence of tokens. The model first projects $\{x_1,...,x_n\}$ to a list of hidden states $\{h_1,...,h_n\}$. Afterwards, ${\{y_1,...,y_m\}}$ can be sequentially decoded from the hidden states.


==> tab-ratio.tex <==
% \begin{table}[h]
%     \centering
%     \begin{tabular}{rlll}
%     \toprule
%      & set 1 & set 2 & set 3 \\
%      \midrule
%     0\% & 7e-1 & 4e-1 & 5e-1 \\
%     20\% & 3e-9 &  8e-8 & 1e-10 \\
%     40\% & 1e-10 & 3e-8 & 5e-11 \\
%     60\% & 1e-9 & 2e-8 & 2e-11 \\
%     80\% & 4e-10 & 7e-9 & 5e-11\\
%     100\% & 1e-9& 2e-8 & 1e-9\\
%     \bottomrule
%     \end{tabular}
%     \caption{p-value of our watermarking approach under various percentages of WMT14 data, which is from the watermarked translation of the victim model.}
%     \label{tab:dff_ratio}
% \end{table}


\begin{table}[h]
    \centering
    %\vspace{-2mm}
    \scalebox{0.83}{
    \begin{tabular}{rrrrrr}
    \toprule
    Percent. & 0\% & 5\% &  10\% & 20\% & 100\%\\
     \midrule
    p-value &0.4641 & 0.0090 &  $<10^{-6}$ & $<10^{-8}$ &  $<10^{-8}$\\
    p-value &0.7237 & 0.2888 &  0.0768 & 0.0087 &  $<10^{-4}$\\
    \bottomrule
    \end{tabular}
    }
    %\vspace{-2mm}
    \caption{p-value of our watermarking approach with different percentages of WMT14 data, which is from the watermarked translation of the victim model.}
    \label{tab:dff_ratio}
    %\vspace{-5.0mm}
\end{table}
